Bayesian Mechanism Design for Budget-Constrained Agents

We study Bayesian mechanism design problems in settings where agents have budgets. Specifically, an agent's utility for an outcome is given by his value for the outcome minus any payment he makes to the mechanism, as long as the payment is below his budget, and is negative infinity otherwise. This discontinuity in the utility function presents a significant challenge in the design of good mechanisms, and classical "unconstrained" mechanisms fail to work in settings with budgets. The goal of this paper is to develop general reductions from budget-constrained Bayesian MD to unconstrained Bayesian MD with small loss in performance. We consider this question in the context of the two most well-studied objectives in mechanism design---social welfare and revenue---and present constant factor approximations in a number of settings. Some of our results extend to settings where budgets are private and agents need to be incentivized to reveal them truthfully.

==> abstract.tex <==
We study Bayesian mechanism design problems in settings where
agents have budgets. Specifically, an agent's utility for an outcome
is given by his value for the outcome minus any payment he makes to
the mechanism, as long as the payment is below his budget, and is
negative infinity otherwise. This discontinuity in the utility
function presents a significant challenge in the design of good
mechanisms, and classical ``unconstrained'' mechanisms fail to work in
settings with budgets. The goal of this paper is to develop general
reductions from budget-constrained Bayesian MD to unconstrained
Bayesian MD with small loss in performance. We consider this question
in the context of the two most well-studied objectives in mechanism
design---social welfare and revenue---and present constant factor
approximations in a number of settings. Some of our results extend to
settings where budgets are private and agents need to be incentivized
to reveal them truthfully.


==> arxiv-intro.tex <==
%(Outline follows.)

Auction and mechanism design have for the most part focused on agents
with quasilinear utility functions: each agent is described by a
function that assigns values to possible outcomes, and the agent's
utility from an outcome is her value minus any payment that she makes
to the mechanism. This implies, for example, that an agent offered an
outcome at a price below her value for the outcome should in the
absence of better alternatives immediately accept that outcome. This
simple model fails to capture a basic practical issue---agents may not
necessarily be able to afford outcomes that they value highly. For
example, most people would value a large precious stone such as the
Kohinoor diamond at several millions of dollars (for its resale value,
if not for personal reasons), but few can afford to pay even a
fraction of that amount. Many real-world mechanism design scenarios
involve financially constrained agents and values alone fail to
capture agents' preferences. Budget constraints have frequently been
observed in FCC spectrum auctions~\cite{BL-09,CG-98}, Google's auction
for TV ads~\cite{Nisan-Google-TV}, and sponsored search auctions, to
take a few examples.

From a theoretical viewpoint, the introduction of budget constraints presents a challenge in mechanism
design because they make the utility of an agent nonlinear and
discontinuous as a function of the agent's payment---the utility
decreases linearly with payment while payment stays below the budget,
but drops to negative infinity when the payment crosses the
budget. The assumption of linearity in payments (i.e. quasilinearity
of utility) underlies much of the theoretical framework for mechanism
design. Consequently, standard mechanisms such as the VCG mechanism
can no longer be employed in settings involving budgets.

The goal of this paper is to develop connections between
budget-constrained mechanism design and the well-developed theory of
unconstrained mechanism design. Specifically we ask ``when can
budget-constrained mechanism design be reduced to unconstrained
mechanism design with some small loss in performance?'' We consider
this question in the context of the two most well-studied objectives
in mechanism design---social welfare and revenue. Some of our results
assume that the mechanism knows the budgets of the agents, but others
hold even when budgets are private and agents need to be incentivized
to reveal them truthfully.

Recent work in computer science has begun exploring a theory of
mechanism design for budget-constrained agents (see, for example,
\cite{Abrams06, BCIMS05, DNL08, CDG10, AJM10}). Most of this work has focused
on {\em prior-free} or worst-case settings, where the mechanism
designer has no information about agents' preferences. Unsurprisingly,
the mechanism designer has very little power in such settings, and
numerous impossibility results hold. For example, in the worst-case
setting no truthful mechanism can obtain a non-trivial approximation
to social welfare~\cite{BCIMS05}. The goal of achieving good social
welfare has therefore been abandoned in favor of weaker notions such
as Pareto optimality~\cite{DNL08}. For the revenue objective while
approximations can be achieved in simple enough settings,
e.g. multi-unit auctions~\cite{BCIMS05}, hardness results hold for
more general feasibility constraints even in the absence of
budgets. In this paper, we sidestep these impossibility results by
considering Bayesian settings where the mechanism designer has prior
information about the distributions from which agents' private values
and private budgets are drawn.

We restrict our attention to direct revelation truthful
mechanisms. Our mechanisms are allowed to randomize, and agents'
utilities are computed in expectation over the randomness used by the
mechanism. As is standard, we assume that both the mechanism and the
agents possess a common prior from which values are drawn. While we
optimize over the class of Bayesian incentive compatible (BIC)
mechanisms, all of the mechanisms we develop are dominant strategy
incentive compatible (DSIC) (see, for example,~\cite{AGT-N} for
definitions of these solution concepts).

In addition, we require that our mechanisms satisfy the ex-post
individual rationality (EPIR) constraint, namely that the payment of
any agent never exceeds her value for the mechanism's outcome. This
implies, in particular, that the mechanism cannot charge any agent to
whom no item or service is allocated. In contrast, most previous work
has enforced the individual rationality constraint only in expectation
over the mechanism's randomness as well as the randomness in other
agents' values (i.e. interim IR).

%%  In Bayesian
%% settings, truthfulness can be achieved to different extents. We
%% consider the following classes of mechanisms:
%% \begin{itemize}
%% \item{\bf Bayesian Incentive Compatible (BIC).} In these mechanisms,
%%   the expected utility of an agent, with the expectation taken over
%%   the mechanism's randomness as well as the randomness in other
%%   agents' values, is maximized when the agent truthfully reports her
%%   type (value as well as budget, when budgets are private). This is
%%   also called interim IC.
%% \item{\bf Dominant Strategy Incentive Compatible (DSIC).} In these
%%   mechanisms, for every setting of other agents' values, an agent's
%%   expected utility, with the expectation taken over the mechanism's
%%   randomness, is maximized when the agent truthfully reports her
%%   type. This is also called ex post IC.
%% \item{\bf Interim IR (IIR).} In these mechanisms, the expected payment
%%   of an agent, with the expectation taken over the mechanism's
%%   randomness as well as the randomness in other agents' values, is no
%%   more than her value. Therefore, her expected utility is non-negative.
%% \item{\bf Ex post IR (EPIR).} In these mechanisms, the actual payment
%%   of an agent is no more than her value, regardless of the draws of
%%   other agents' values or the mechanism's coin flips. Therefore, her
%%   utility is non-negative with probability $1$.
%% \end{itemize}

%% Clearly DSIC is a stronger constraint than BIC and EPIR is a stronger
%% constraint than IIR. Note that the EPIR constraint is quite similar to
%% the budget constraint, which is also an ex post constraint that must
%% be satisfied with probability $1$. In general our goal is to design
%% DSIC EPIR mechanisms that achieve approximate-optimality for our
%% objectives with respect to optimal BIC EPIR mechanisms.

It is worth noting here that the EPIR constraint is not without loss
in performance. Consider the following example: suppose we are selling
a single item to one of $n$ agents, each with a value of $v$ with
probability $1$ (that is publicly known) and a public budget of $v/n$
with probability $1$. Now, under the IIR constraint, the optimal
auction asks agents to pay what they bid and offers each agent that
pays at least $v/n$ a fair chance at winning the item. Each agent pays
$v/n$, the item is allocated to a random agent, and the mechanism's
revenue is $v$. Under the EPIR constraint, however, a mechanism can
only charge the agent that wins the item and can charge this agent no
more than $v/n$. As we can see, the revenue gap between the optimal
IIR and the optimal EPIR mechanism gets larger and larger as $n$ grows.

It is well known that over the class of BIC IIR mechanisms,
the revenue-optimal as well as welfare-optimal mechanisms are both
so-called ``all-pay'' auctions \cite{M00,PV08}.  In all-pay auctions
agents pay the mechanism a certain (distribution dependent) function
of their value regardless of the allocation that the mechanism
makes. The optimality of all-pay auctions follows by noting that
any allocation rule that admits some BIC budget-feasible payment
function can be implemented with an all-pay payment rule with
worst-case payments that are no larger than those in any other
truthful payment rule and are therefore budget-feasible.
Unfortunately all-pay auctions have many undesirable properties. In
many settings it is simply not feasible to force the agents to pay
upfront without knowing the outcome of the mechanism. Moreover all-pay
auctions may admit many Bayes-Nash equilibria (BNE), truthtelling
being merely one of them. %% \footnote{For an example, consider a
%% single-item auction with two agents, both of whose values are
%% distributed independently and uniformly over $[0,1]$. Consider an
%% all-pay mechanism that asks agents to report bids, pay their bids, and
%% then allocates the item to the highest bidder. This mechanism admits a
%% continuum of equilibria parameterized by $c\in [1/2,2]$, where agent 1
%% bids $b_1(v_1) = cv_1^2/2$ and agent 2 bids $b_2(v_2) = v_2^2/2c$. The
%% symmetric equilibrium with $c=1$ corresponds to the same allocation
%% rule as the Vickrey auction, and therefore admits truthtelling as a
%% BNE if implemented as a direct revelation mechanism. In contrast,
%% second price auctions are always DSIC, and first-price auctions
%% typically admit a unique BNE~\cite{leb-04}.}
Then the fact that a certain objective is achieved when all the agents
report their true types does not necessarily imply that the objective
will be achieved in practice if a different BNE gets played
out. Therefore, in a departure from previous work, we choose to
enforce ex-post individual rationality.

%% Most previous work on budget-constrained Bayesian MD has focussed on
%% all-pay auctions. Define. Indeed, any truthful allocation rule can be
%% implemented with an all-pay payment rule, with payments no larger than
%% any other truthful payment rule, and therefore budget-feasible. This
%% implies that in general the optimal budget-constrained auction is an
%% all-pay auction. In a departure from this conventional approach, we
%% design (randomized, in expectation over the mechanism's randomness)
%% DSIC mechanisms. All-pay auctions are often unnatural. Moreover, even
%% in the simplest settings, they typically admit many BNE (give
%% example). While previous work claims to obtain truthful all-pay
%% mechanisms, in fact, they merely show that truthtelling is one (of
%% many possible) BNE. This makes all their claims about the mechanism's
%% performance suspect. Note the difference between ex-post and interim
%% IR, and that again, the optimal ex-post IR mechanism may be strictly
%% worse than the optimal interim IR one.

\subsection*{Our results and techniques}

%% Our approximation guarantees depend on several parameters: whether the
%% budgets are public knowledge or private, the feasibility constraint
%% faced by the seller (e.g. a supply constraint), whether the agents'
%% values are single-dimensional (agent $i$'s value for any outcome is
%% either $\vali$ or $0$) or multi-dimensional (agent $i$ may value
%% different outcomes at different levels), and the distributions of the
%% agents' values.

We begin our investigation with the revenue objective and give an
exact characterization of the optimal mechanism for a single agent
with a public budget. While in the absence of budgets the optimal
mechanism is a fixed sale price and therefore deterministic, with
budgets the optimal mechanism may need to randomize and offer multiple
buying options to the agent. This complicates the design of optimal
mechanisms in more general settings involving multiple agents or
private budgets. We therefore consider approximations. When budgets
are known publicly, we obtain constant factor approximations in nearly
all settings where constant factor approximations are known for
unconstrained mechanism design. This includes, for example, all
single-parameter settings with a downwards closed feasibility
constraint, but also multi-parameter settings with ``unit-demand''
agents and a matroid feasibility constraint (see,
e.g., \cite{CHMS10}). Our mechanisms are for the most part direct
reductions to unconstrained settings, and are extremely simple.

For private budgets, the problem becomes much harder and we focus on
settings with single-dimensional values. 
%% We present a general characterization of mechanisms that are 
%% truthful for both values and budgets. We use this to 
We design a novel mechanism based on
``lotteries'' that obtains a good approximation whenever each agent's
value distribution satisfies the monotone hazard rate (MHR) condition
(see Section~\ref{sec:def} for a definition). Our mechanism's novelty
lies in offering each agent a carefully constructed set of different
buying options such that the best option for the agent is to either
spend his entire budget or a fraction of the monopoly price for that
agent. The MHR assumption is a frequently used assumption in mechanism
design literature and many natural distributions satisfy it. In fact
the mechanism obtains a good approximation more generally under mild
technical conditions on the values and budgets. We believe that our
techniques should extend to provide good approximations for arbitrary
distributions.

Next we examine the welfare objective. While for revenue, the budget
of an agent is a natural upper bound on the contribution of that agent
to the revenue and allows us to ``cap'' values at the budget, for
welfare this doesn't work. In fact, a mechanism can generate a
non-trivial guarantee on welfare even when budgets are $0$. Consider a
setting with two unit demand buyers and two items.  Consider the
following mechanism: the mechanism asks each agent to give a
preference list of the items. If the top choices of the buyers are
different, then each buyer gets allocated his top choice and welfare
is maximized. Otherwise, the mechanism ignores the preferences of the
buyers and computes the allocation that maximizes the social welfare
ex-ante. Note that this mechanism is truthful. When agents' values for
the items are i.i.d., the obtained social welfare from this example is
at least $3/4$ of the maximum social welfare we can obtain with no
budget constraint. On the other hand, a mechanism that ``ignores''
values above the budget (i.e. does not distinguish between them in the
allocation function) cannot obtain an approximation better than
$1/2$. The gap between the two mechanisms increases as the number of
agents grows.

We again focus on single-parameter settings and public budgets, but
with arbitrary downwards closed feasibility constraints. For these
settings, we show a tradeoff between an approximation on budget and an
approximation on welfare: for any $\epsilon$, we can get a $1/\eps$
approximation to welfare with respect to the welfare that an optimal
mechanism can get when budgets are scaled down by a factor of
$1-\eps$. This mechanism has an extremely simple form: it replaces
every value larger than its budget by its expectation conditioned on
being larger than the budget, and runs the VCG mechanism on these
modified values. Moreover, if we are willing to sacrifice EPIR in
favor of the less restrictive IIR, we can convert this mechanism into
a 4-approximate IIR mechanism (with no approximation on budgets).

Finally, if the value distributions satisfy the MHR condition, we
achieve a $2(1+e)$-approximation to welfare via an EPIR mechanism by
reducing budget-feasible welfare maximization to budget-feasible
revenue maximization.

One nice property of our reductions from budget feasible mechanism
design to unconstrained mechanism design is that they are for the most
part oblivious to the feasibility constraint imposed on the
mechanism. They therefore work for a broad range of feasibility
constraints and add minimal complexity to the mechanism design
problem.  

%The mechanisms we design are simple, intuitive, and easy to implement.


\subsection*{Related work}


Several works in economics have studied characterizations of optimal
BIC IIR budget-feasible mechanisms (e.g., \cite{PV08, LR96, CG2000,
M00}). However, these works are generally weak in the kinds of
settings they consider (typically just single-item auctions) and the
kinds of value distributions they allow\footnote{E.g., \cite{PV08}
and \cite{M00} make the assumption that value distributions have a
monotone hazard rate as well as a nondecreasing density function,
unnatural conditions that few distributions satisfy simultaneously.}.
Laffont and Robert \cite{LR96} considered single item settings where
bidders have a private value and public common budget. Che and
Gale~\cite{CG2000} considered the setting with a single item and a
single buyer, but allowed both the value and the budget to be
private. Pai and Vohra~\cite{PV08} gave a more general result in which
they designed an optimal auction for a single item and multiple buyers
with private i.i.d. values and private budgets.


%% Bayesian mechanism design widely studied in economics literature. A
%% common motivated objective functions in this setting, is revenue
%% maximization. However most of the existing literature is focused on
%% single dimensional setting. Myerson \cite{mye-81}, solved the revenue
%% maximization problem in this setting for single item with no budget
%% constraint. He also present a complete characterization of incentive
%% compatible mechanisms in the same setting. Based on his
%% characterization, for any incentive compatible mechanism, the
%% allocation rule should be monotone.  Also, he showed how to compute
%% the payments based on an specified monotone allocation rule. When
%% budget constraint is added to the setting, we no longer can use his
%% approach for maximizing revenue since some of the payments might not
%% satisfy the budget constraint. Chawla et al
%% \cite{CHMS10},\cite{CHK07}, considered the multidimensional setting
%% with unit demand buyers without budget constraint and studied the
%% revenue maximizing objective function in Bayesian setting. They
%% designed a sequential posted price mechanism and showed that their
%% mechanism obtains constant approximation of the optimal.

%% The existing literature on mechanism design with budget constraint
%% looked at both objectives of social welfare as well as Revenue
%% maximization. These objectives have been studied from two
%% perspectives: prior free setting and Bayesian setting.

Bhattacharya et al.~\cite{BGGM10} were the first to study settings
beyond single-item auctions and focused on revenue maximization. They
considered a setting with heterogeneous items and additive values, and
exhibited a (large) constant factor DSIC approximation mechanism as
well as an all-pay auction which admits truthtelling as a BNE and in
that BNE obtains a $4$-approximation. However, these results required
the value distributions to satisfy the MHR condition. The mechanisms
are LP-based. In contrast most of our mechanisms are easy to compute,
work for general distributions, enforce EPIR, and achieve small
approximation factors.

%% showed that if the
%% type space of each buyer is a product distribution that satisfies the
%% monotone hazard condition, their sequential posted pricing mechanism
%% obtains a constant approximation compared to the revenue of the
%% optimal ex post truthful mechanism, and also presented an all-pay
%% auction which admits truthtelling as a BNE and in that BNE obtains a
%% $4$-approximation.

In prior-free settings few results are known for revenue
maximization. Borgs et al.~\cite{BCIMS05} looked at multi unit
auctions for homogeneous goods where agents have private values and
budgets and considered worst case competitive ratio (see
also \cite{Abrams06}). They designed a mechanism based on random
sampling that maximizes revenue when the number of bidders is large.

Social welfare maximization has also been considered under budget
constraints. Maskin~\cite{M00} considered the setting of a single item
and multiple buyers with public budgets. He defined and showed how to
compute the constrained efficient mechanism, the truthful feasible
mechanism under budget constraints that maximizes the expected social
welfare (however, the result holds only for some distribution
functions \cite{PV08}). In prior-free settings for multi unit
homogeneous items, Nisan et al.~\cite{DNL08} studied Pareto efficient
DSIC mechanisms with budget constraints. They showed that if the
budgets are private there is no Pareto optimal incentive compatible
mechanism; for public budgets they showed that there exists a unique
mechanism based on the \emph{clinching auction}. Chen et al.~\cite{CDG10}
considered a setting with multiple goods and unit demand buyers and
showed how to compute competitive prices that enforce truthfulness
under budget constraints if such prices exist. Finally, the work of
Alaei et al.~\cite{AJM10} stands out in their study of ``soft''
budgets constraints, where buyers pay an increasing interest rate for
payments made above their budgets. They showed how to exactly compute
the smallest competitive prices in this setting that result in an
incentive compatible mechanism with an outcome in the core.



%\begin{itemize}
%\item
%Social Welfare maximization
%\item
%Revenue maximization
%\end{itemize}
%and each category has been studied under two common models:
%\begin{itemize}
%\item
%Bayesian setting
%\item
%Prior free setting
%\end{itemize}
%
%Kamesh et al: considered heteregeneous items with additive values and budget constraint. The
%mechanism is based on all pay auction and they get a 4 approximation. for the case of iid they gave
%O(1) approximation for monotone hazard rate for expost incentive compatibility.
%
%Laffont and Robert: Revenue maximizing, single item, public common budget.BIC
%
%Che and Gale considered revenue maximizing when there is a single buyer with value and budget
%private.
%
%Rakesh and mallesh: types are iid where type is two tuple and value and budget with monotone hazard
%rate, n bidders with private budgets
%\item Non-Bayesian
%Borgs et al looked at multi unit auction and considered worst case competitive ratio and design a
%mechanism that maximizes revenue when the number of bidders is large.
%\end{itemize}
%\item
%Social welfare
%\begin{itemize}
%\item
%Bayesian: maskin looked at efficiency single item bayesian setting with public budgets(possibly
%different) and computed the constrained efficient mechanism for liquidity constrained bidders. BIC
%\item
%Non-bayesian Nisan et al for multi unit auction with private budgets showed that there is no pareto
%optimal incentive compatible mechanism and for public auction they showed there is a unique
%solution that can compute the pareto optimal incentive compatible outcome.
%\end{itemize}
%\end{itemize}
%\end{itemize}
%
%With no budgets: Shuchi paper for unit demand single buyer and the general setting for revenue
%maximization in unit demand setting in multidimensional setting.
%
%Rakesh paper: looked at hard budget constraint: symmetric revenue maximizing and constrained
%efficient auctions in this setting when both value and budget are private information. Here there
%is only one item to sell. The auction is in all pay format.
%
%Che and Gale: Revenue ranking between different auctions
%
%
% Problem of maximizing efficiency and revenue without budget constraint is very well
%studied in economics literature. If there is no budget constraint, VCG mechanism gives the optimal
%truthful mechanism and it is computable in polynomial time for single item and unit demand bidders.
%However, if bidders have budget constraints, the VCG might not be implementable anymore.
%
%
%
% Azarakhsh: this will need work from you.
%
%As mentioned earlier, much work has focused on all-pay
%mechanisms. These are undesirable.
%
%Other results make unnatural assumptions on the distribution:
%MHR. This is unrealistic, for example, doesn't allow bimodal
%distributions. Another unrealistic assumption found commonly: f(v) is
%increasing.
%
%Review work on soft budgets
%
%Review work on worst-case budget-constrained settings


==> macros.tex <==
%counters for theorem numbers
\newcounter{temp}
\newcounter{myeCount}
\newcounter{myeVsSumPqCount}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}{Example}
%\newcommand{\qed}{\mbox{\ \ \ }\rule{6pt}{7pt} \bigskip}
%\newcommand{\mathqed}{\mbox{\ \ \ \rule{6pt}{7pt}}}
\renewcommand{\comment}[1]{}
%\newenvironment{proof}{\noindent{\em Proof:}}{\hfill\qed}
\newenvironment{proofsketch}{\noindent{\em Proof Sketch:}}{\qed}
\newenvironment{proofof}[1]{\noindent{\em Proof of #1.}}{}

%\newcommand{\argmax}{{\text {argmax}}}
%\newcommand{\argmin}{{\text {argmin}}}
\newcommand{\argmax}{\operatorname{argmax}}
\newcommand{\argmin}{\operatorname{argmin}}
\DeclareMathOperator*{\E}{E}
\DeclareMathOperator*{\argminLoglike}{argmin}
\DeclareMathOperator*{\argmaxLoglike}{argmax}

\newcommand{\poly}{{\text {poly }}}


\newcommand{\groundset}{J}


\newcommand{\A}{{\mathcal A}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\OPT}{{\mbox {OPT}}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\iid}{{i.~i.~d.\ }}

\newcommand{\val}{v}
\newcommand{\vals}{{\mathbf \val}}
\newcommand{\valsmi}{{\mathbf \val}_{-i}}
\newcommand{\valsmij}{{\mathbf \val}_{-ij}}
\newcommand{\vali}[1][i]{{\val_{#1}}}
\newcommand{\valj}[1][j]{{\val_{#1}}}
\newcommand{\valij}[1][ij]{{\val_{#1}}}


\newcommand{\partition}{J}
%\newcommand{\parts}{{\mathbf \partition}}
\newcommand{\parts}{\Pi}
\newcommand{\parti}[1][i]{{\partition_{#1}}}


\newcommand{\bid}{b}
\newcommand{\bids}{{\mathbf \bid}}
\newcommand{\bidi}[1][i]{{\bid_{#1}}}

\newcommand{\virt}{\phi}
\newcommand{\virts}{{\mathbf \virt}}
\newcommand{\virti}[1][i]{{\virt_{#1}}}
\newcommand{\vopt}{\val^{\ast}}

\newcommand{\virtinv}{\virt^{-1}}
\newcommand{\virtiinv}[1][i]{\virt_{#1}^{-1}}
\newcommand{\virtval}{\nu}

\newcommand{\ivirt}{\bar{\virt}}
\newcommand{\ivirtinv}{\ivirt^{-1}}
\newcommand{\ivirtiinv}{\ivirt_i^{-1}}
\newcommand{\ivirti}[1][i]{{\ivirt_{#1}}}

\newcommand{\vmin}{\ell}
\newcommand{\vmax}{h}

\newcommand{\dist}{F}
\newcommand{\dists}{{\mathbf \dist}}
\newcommand{\disti}[1][i]{{\dist_{#1}}}
\newcommand{\distj}[1][j]{{\dist_{#1}}}
\newcommand{\distij}[1][ij]{{\dist_{#1}}}

\newcommand{\dens}{f}
\newcommand{\denss}{{\mathbf \dens}}
\newcommand{\densi}[1][i]{{\dens_{#1}}}
\newcommand{\densj}[1][j]{{\dens_{#1}}}

\newcommand{\price}{p}
\newcommand{\prices}{{\mathbf \price}}
\newcommand{\pricei}[1][i]{{\price_{#1}}}
\newcommand{\pricej}[1][j]{{\price_{#1}}}
\newcommand{\priceij}[1][ij]{{\price_{#1}}}
\newcommand{\pricemi}[1][i]{{\price^M_{#1}}}
\newcommand{\pricemj}[1][j]{{\price^M_{#1}}}
\newcommand{\pricesi}[1][i]{{\price^S_{#1}}}
\newcommand{\rightpeakpricei}{\overline{\pricei}}
\newcommand{\leftpeakpricei}{\underline{\pricei}}

\newcommand{\rprice}{p}
\newcommand{\rprices}{{\mathbf \rprice}}
\newcommand{\rpricei}[1][i]{{\rprice_{#1}}}

\newcommand{\prob}{x}
\newcommand{\probs}{{\mathbf \prob}}
\newcommand{\probi}[1][i]{{\prob_{#1}}}
\newcommand{\probj}[1][j]{{\prob_{#1}}}
\newcommand{\probmi}[1][i]{{\prob^M_{#1}}}
\newcommand{\probmj}[1][j]{{\prob^M_{#1}}}
\newcommand{\probsi}[1][i]{{\prob^S_{#1}}}
\newcommand{\rightpeakprobi}{\overline{\probi}}
\newcommand{\leftpeakprobi}{\underline{\probi}}

\newcommand{\Mye}{\mathcal M}
\newcommand{\Alg}{\mathcal A}
%\newcommand{\vcg}[1][]{{\mathcal V}^{#1}}
\newcommand{\I}{\mathcal I}

\newcommand{\Rev}{{\mathcal R}}
\newcommand{\RevMye}{\Rev^{\Mye}}
\newcommand{\RevAlg}[1][\Alg]{\Rev^{#1}}
\newcommand{\Revp}[1][\prices]{\Rev^{#1}}

\newcommand{\sets}{\mathcal{S}}

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\spanOf}{\operatorname{sp}}
\newcommand{\spanOfBrief}{\operatorname{sp}}
\newcommand{\MISpanOf}{\operatorname{MISpan}}
\newcommand{\vsurp}{\Phi}
\newcommand{\cost}{\kappa}
\newcommand{\sv}{{\text{sv}}}

%FIXME: not sure this looks very good...
\newcommand{\expect}{\mathop{\operatorname{E}}}
\newcommand{\pr}{\mathop{\operatorname{Pr}}}
\newcommand{\abs}[1]{\lvert{#1}\rvert}



%budgets related defs

\newcommand{\mech}{M}
\newcommand{\spm}{{\mathbf S}}
\newcommand{\alloc}{x}
\newcommand{\allocs}{{\mathbf \alloc}}
\newcommand{\alloci}[1][i]{\alloc_{#1}}
\newcommand{\allocj}[1][j]{\alloc_{#1}}
\newcommand{\allocij}[1][ij]{\alloc_{#1}}
\newcommand{\Ifc}{\I^\text{reps}}
\newcommand{\Imin}{\widehat{\I}}
\newcommand{\Iminfc}{{\Imin}^\text{reps}}

\newcommand{\distb}{G}
\newcommand{\distbs}{{\mathbf \distb}}
\newcommand{\distbi}[1][i]{{\distb_{#1}}}
\newcommand{\distbj}[1][j]{{\distb_{#1}}}


\newcommand{\distmin}{\widehat{\dist}}
\newcommand{\distmins}{{\mathbf \distmin}}
\newcommand{\distmini}[1][i]{{\distmin_{#1}}}
\newcommand{\distminj}[1][j]{{\distmin_{#1}}}
\newcommand{\distminij}[1][ij]{{\distmin_{#1}}}
\newcommand{\mechmin}{\widehat{\mech}}

\newcommand{\valmin}{\hat{\val}}
\newcommand{\valmins}{{\mathbf \valmin}}
\newcommand{\valminsmi}{{\mathbf \valmin}_{-i}}
\newcommand{\valmini}[1][i]{{\valmin_{#1}}}
\newcommand{\valminj}[1][j]{{\valmin_{#1}}}
\newcommand{\valminij}[1][ij]{{\valmin_{#1}}}

\newcommand{\allocmin}{\hat{\alloc}}
\newcommand{\allocmins}{{\mathbf \allocmin}}
\newcommand{\allocmini}[1][i]{\allocmin_{#1}}
\newcommand{\allocminj}[1][j]{\allocmin_{#1}}
\newcommand{\allocminij}[1][ij]{\allocmin_{#1}}

\newcommand{\pricemin}{\hat{\price}}
\newcommand{\pricemins}{{\mathbf \pricemin}}
\newcommand{\pricemini}[1][i]{\pricemin_{#1}}
\newcommand{\priceminj}[1][j]{\pricemin_{#1}}
\newcommand{\priceminij}[1][ij]{\pricemin_{#1}}

\newcommand{\budget}{B}
\newcommand{\budgets}{\mathbf{\budget}}
\newcommand{\budgetsmi}{\mathbf{\budget}_{-i}}
\newcommand{\maxBudget}{\widehat{\budget}}
\newcommand{\maxBudgeti}[1][i]{\maxBudget_{#1}}
\newcommand{\budgeti}[1][i]{\budget_{#1}}
\newcommand{\budgetj}[1][j]{\budget_{#1}}

\newcommand{\bgtSet}{\mathcal{B}}
\newcommand{\vickSet}{\mathcal{A}}
\newcommand{\lowSet}{L}
\newcommand{\highSet}{H}
\newcommand{\bgtMech}{\mech_{\bgtSet}}

\newcommand{\lparam}{\alpha}
\newcommand{\lparamOpt}{\lparam^{\ast}}
\newcommand{\lotto}[1][\lparam]{\ell_{#1}}
\newcommand{\lThresh}{T}
\newcommand{\lThreshi}[1][i]{\lThresh_{#1}}
\newcommand{\lottos}[1][\maxBudget,\lThresh]{\mathcal{L}({#1})}
\newcommand{\lottosi}[1][\maxBudgeti,\lThreshi]{\lottos{#1}}

%defs for the single agent optimal proof
\newcommand{\iprob}{\tilde{\prob}}
\newcommand{\probSet}{\mathcal{A}}
\newcommand{\probSeti}{\widetilde{\probSet}}
\newcommand{\probSetOpt}{\mathcal{A}^{\ast}}
\newcommand{\pmax}{{\prob}_{\text{max}}}
\newcommand{\popt}{{\prob}^{\ast}}
\newcommand{\popti}{{\iprob}^{\ast}}

\newcommand{\g}{g}
\newcommand{\G}{G}
\newcommand{\gi}{\hat{\g}}
\newcommand{\Gi}{\hat{\G}}

\newcommand{\vlo}{\underline{\val}}
\newcommand{\vhi}{\bar{\val}}

%commands for the private budget 2-approx
\newcommand{\minp}{\underline{\price}}
\newcommand{\maxp}{\bar{\price}}

\newcommand{\optS}{\bgtSet}

\newcommand{\lottoMech}{{\mech}^{\mathcal{L}}}
\newcommand{\lottosTarget}[1][\minp,\maxp]{\lottos[{#1}]}
\newcommand{\revFromOptS}{\RevAlg[\mech\cap\optS]}
\newcommand{\revNotOptS}{\RevAlg[\mech\setminus\optS]}


%\newcommand{\fixme}[1]{\noindent\framebox[6.5in]{\hfill\parbox{.75in}{\em FIXME:}\hfill\parbox{5.5in}{#1}}\par}
\newcommand{\fixme}[1]{}

